Real-Time Radiance Fields for Single-Image Portrait View Synthesis

We present a one-shot method to infer and render a photorealistic 3D representation from a single unposed image (e.g., face portrait) in real-time. Given a single RGB input, our image encoder directly predicts a canonical triplane representation of a neural radiance field for 3D-aware novel view synthesis via volume rendering. Our method is fast (24 fps) on consumer hardware, and produces higher quality results than strong GAN-inversion baselines that require test-time optimization. To train our triplane encoder pipeline, we use only synthetic data, showing how to distill the knowledge from a pretrained 3D GAN into a feedforward encoder. Technical contributions include a Vision Transformer-based triplane encoder, a camera data augmentation strategy, and a well-designed loss function for synthetic data training. We benchmark against the state-of-the-art methods, demonstrating significant improvements in robustness and image quality in challenging real-world settings. We showcase our results on portraits of faces (FFHQ) and cats (AFHQ), but our algorithm can also be applied in the future to other categories with a 3D-aware image generator.

==> sections/definitions.tex <==
\newcommand{\model}{$\pi$-GAN\xspace}
\newcommand{\siren}{{\sc siren}}

\newcommand{\pose}{\xi}
\newcommand{\coord}{\mathbf{x}}
\newcommand{\noise}{\mathbf{z}}
\newcommand{\dir}{\mathbf{d}}
\newcommand{\density}{\sigma}
\newcommand{\col}{\mathbf{c}}

\newcommand{\generatorparams}{\theta_G}
\newcommand{\generator}{G_{\generatorparams}}
\newcommand{\discriminatorparams}{\theta_D}
\newcommand{\discriminator}{D_{\discriminatorparams}}

\newcommand{\filmmult}{\boldsymbol{\gamma}}
\newcommand{\filmadd}{\boldsymbol{\beta}}

\newcommand{\implicitlayer}{\phi}
\newcommand{\implicit}{\Phi}
\newcommand{\implicitparams}{\theta}
\newcommand{\nonlinearlayer}{\sin}

\newcommand*\rot{\rotatebox{90}}




\newif\ifdrafting
\draftingtrue %

\ifdrafting
    \newcommand{\mc}[1]{\textcolor{magenta}{[Matthew: #1]}}
    \newcommand{\rr}[1]{\textcolor{blue}{[Ravi: #1]}}
    \newcommand{\alex}[1]{\textcolor{green}{[Alex: #1]}}
    \newcommand{\kn}[1]{\textcolor{red}{[Koki: #1]}}
    \newcommand{\zy}[1]{\textcolor{orange}{[Zhiding: #1]}}
\else
    \newcommand{\mc}[1]{}
    \newcommand{\rr}[1]{}
    \newcommand{\alex}[1]{}
    \newcommand{\kn}[1]{}
    \newcommand{\zy}[1]{}
\fi


